Adaptive 3D-IC TSV Fault Tolerance Structure Generation

In three dimensional integrated circuits (3D-ICs), through silicon via (TSV) is a critical technique in providing vertical connections. However, the yield and reliability is one of the key obstacles to adopt the TSV based 3D-ICs technology in industry. Various fault-tolerance structures using spare TSVs to repair faulty functional TSVs have been proposed in literature for yield and reliability enhancement, but a valid structure cannot always be found due to the lack of effective generation methods for fault-tolerance structures. In this paper, we focus on the problem of adaptive fault-tolerance structure generation. Given the relations between functional TSVs and spare TSVs, we first calculate the maximum number of tolerant faults in each TSV group. Then we propose an integer linear programming (ILP) based model to construct adaptive fault-tolerance struc- ture with minimal multiplexer delay overhead and hardware cost. We further develop a speed-up technique through efficient min-cost-max-flow (MCMF) model. All the proposed method- ologies are embedded in a top-down TSV planning framework to form functional TSV groups and generate adaptive fault- tolerance structures. Experimental results show that, compared with state-of-the-art, the number of spare TSVs used for fault tolerance can be effectively reduced.

==> doc/answer.tex <==
{

\onecolumn
\normalsize

\ \\
\textbf{Responses to reviewers}

\ \\
\textbf{Reviewer 1}
\begin{description}\itemsep.8em

\item[R1C1]
First, in my opinion, the novelty of the problem under investigation and the proposed technique is not strong enough. In the revision, the authors only improved the writing and add some new contents.
\item[R1A1]\revise{
Thanks very much for the comments.}
%All previous works (e.g.~\cite{wang2015defect,xu2017clustered}) deals with a special type of TSV fault-tolerance structure generation.
%That is, they are under an assumption that a predetermined number of s-TSVs are assigned to each TSV group, and an f-TSV in a group should be replaced by any s-TSV within the group.
%An example is illustrated in Fig.~\subref*{fig:special:a}, where five f-TSVs ($f_1 \cdots f_5$) and four s-TSVs ($s_1 \cdots s_4$) are in the TSV group.
%Due to unreasonable position of $s_4$, it can only be connected by $f_5$.
%In this case, the previous works cannot generate a fault-tolerance structure that satisfies the chip yield.}

\revise{3D integration has already seen commercial applications in the form of 3D memory but there are still significant open problems in both research and implementation. A sentence is added at the end of the first paragraph in Section \ref{sec:intro}  and one more reference \cite{tcad2017Lu} is added.}

\revise{A paragraph at the end of Section \ref{sec:problem} is added to discuss the forming of TSV groups since the fault-tolerance structure generation involves the forming of TSV groups and the generation of fault-tolerance structures within every TSV group.
In the fourth paragraph of Section \ref{sec:tfts}, we revised the discussion of the generalized example of TSV group.
}

%\revise{
%To ensure the existence of fault-tolerance structures in TSV groups, the previous works \cite{wang2015defect,xu2017clustered} form TSV groups under two constraints: (1) the number of s-TSVs equals the number of tolerable faults and (2) an f-TSV in a group can be replaced by any s-TSV within the group.
%Fig.\subref*{fig:special:a} shows an example of TSV group having two-fault tolerance structures, where all the f-TSVs, $f_1$, $f_2$, $f_3$, and $f_4$, can be replaced by both $s_1$ and $s_2$ considering the net bounding boxes.}
\revise{
Here, we explain our contributions based on the generalized example shown in
Fig.~\subref*{fig:special:a}, where five f-TSVs ($f_1 \cdots f_5$) and four s-TSVs ($s_1 \cdots s_4$) are involved. The replaceable relations between TSVs are shown in Fig.~\subref*{fig:origgraph1}.
The methods in \cite{wang2015defect} cannot generate cost-effective fault-tolerance structures for this TSV group even though the f-TSV group is partitioned into smaller groups, because $f_2$ has no candidate s-TSVs. The ILP-based method in \cite{xu2017clustered} cannot generate fault-tolerance structures for this TSV group since the number of tolerant faults is unknown. However, the f-TSV group definitely includes a two-fault tolerance structure as shown in Fig.~\subref*{fig:origgraph2}, where three out of four s-TSVs are used in the fault-tolerance structure.
%In this case, the previous works cannot generate a fault-tolerance structure that satisfies the chip yield.
}

\revise{
%To address the new design challenging if not all s-TSVs can be occupied in constructing $K$-fault tolerance structure,
In this work, we propose to generate adaptive fault-tolerance structures, in which the number of tolerant faults is adaptively determined by the distribution of the f-TSVs and their candidate s-TSVs. %Key technical contributions of this work are listed as follows.
%\revise{
\begin{itemize}
  \item \textbf{Given the distribution of f-TSVs and their candidate s-TSVs, we are able to determine the maximum number of tolerant faults, denoted as $K$, in polynomial time.} For the TSV group shown in Fig.~\subref*{fig:special:a}, we can determine the maximum number of tolerant faults, $K=2$, by solving a max-flow problem on the splitting graph shown in Fig.~\subref*{fig:splitgraph}.
  \item \textbf{We present an integer linear programming formulation for generating the adaptive $K$-fault tolerance structures}, where both the maximum port number of multiplexers and the number of used s-TSVs are minimized. For the TSV group in Fig.~\subref*{fig:special:a}, the proposed method generates an adaptive fault-tolerance structure as shown in Fig.~\subref*{fig:special:b}, which uses three s-TSVs out of four s-TSVs and can tolerate two TSV faults.
  \item \textbf{We further propose an efficient min-cost-max-flow (MCMF) based heuristic method to speed-up the $K$-fault tolerance structure generation.}
  \item \textbf{All the proposed methodologies are embedded in a top-down TSV planning framework to form f-TSV groups and generate fault-tolerance structures.}  If the target TSV yield is not satisfied, a selected TSV group (generally, the group with the lowest yield) will be partitioned into two new TSV groups. For a new TSV group, we will first determine how many TSV faults can be tolerated in the group and, then, the MCMF-based heuristic will be invoked to allocate s-TSVs.
 With the allocated s-TSVs and the f-TSVs, the chip TSV yield will be re-evaluated. New TSV groups will be iteratively generated until the target TSV yield is satisfied.
\end{itemize}
 %Because of the adaptive fault-tolerance structures, the number of TSV groups is significantly reduced.
 Experimental results show that, the proposed framework can significantly reduce the number of used s-TSVs and maximum port number of multiplexers.
 }


\item[R1C2]
Second, although more thorough experiments are carried out and compared with previous works, the results is based on old and small benchmarks. It's better to use more realistic 3D circuit benchmarks.
\item[R1A2]\revise{
Thanks very much for the great suggestion.
In this revision we adopt one more industrial 2D design, which contains 403266 cells and 448514 nets.
{hMetis} \cite{karypis1999multilevel} is adopted to partition the design into several blocks for floorplanning.
Based on different block numbers, two benchmark cases, \texttt{t337} and \texttt{t469}, are generated.
That is, \texttt{t337} has 337 blocks and 1836 nets, while \texttt{t469} has 469 blocks and 5479 nets.
Since the square has the smallest perimeter among all the rectangles with the same area \cite{chen2008fixed}, here the shapes of all the blocks are set to square.
We have added some explanations in Section \ref{sec:etp} and update experimental results in TABLEs~\ref{tab:tab7}--\ref{tab:tab8}.
}

\end{description}


\ \\
\textbf{Reviewer 2}
\begin{description}\itemsep.8em

\item[R2C1]
Abstract: ``but a legal structure cannot always be found due to unreasonable TSV locations.''
Still not clear enough. Do the authors mean ``feasible (or practical) solution'' by ``legal structure''? What is ``unreasonable TSV location''?
\item[R2A1]\revise{
Thanks very much for the comments. We have revised ``a legal structure'' as ``a valid structure'' and revised the whole sentence as follows.:
``but a valid structure cannot always be found due to the lack of effective generation methods for fault-tolerance structures."}

\revise{In addition, we have added one paragraph in Section \ref{sec:tfts} for more elaborations.}

%\revise{To address the new design challenging, %if not all s-TSVs can be occupied in constructing $K$-fault tolerance structure,
%in this paper, we propose to generate adaptive fault-tolerance structures, in which the number of tolerant faults is
%adaptively determined by the distribution of the f-TSVs and their candidate s-TSVs.
%Fig.~\subref*{fig:special:b} shows an adaptive fault-tolerance structure, which uses three s-TSVs out of four s-TSVs and can tolerate two TSV faults.
%}

\item[R2C2]
Page 11, Column1, Line 29: ``... the TSV defect probability $p$ is set to 0.001''
What is this choice of $p$ based on? Are there any references that this is a typical TSV defect probability? Otherwise, it might be good to use multiple values within a reasonable range of $p$.
\item[R2A2]\revise{
Thanks very much for the comments. The TSV defect probability $p$ in~\cite{jiang2012effective} ranges from 0.001 to 0.01.
In the revised manuscript, we also execute the experiment when $p$ is set to 0.01 under 3-fault tolerance structures.
Each benchmark case is executed 20 times independently.
We have added the experimental results in TABLE~\ref{tab:tab10}.
}

\item[R2C3]
Abstract: ``additional spare TSV'' -- I suggest to remove ``additional'', as it is implied by ``spare''.
\item[R2A3]\revise{
Thanks very much for the comments. We have updated the abstract accordingly.
}
\end{description}


\ \\
\textbf{Reviewer 3}
\begin{description}\itemsep.8em

\item[R3C1]
Please add a small discussion that describes the limitations of your methodology.
\item[R3A1]\revise{
Thanks very much for the comments. In this work, the proposed TSV fault tolerance planning is performed in the floorplanning stage and
it is difficult to obtain accurate wire delay information. Therefore, we use the half-perimeter wirelength to reflect the wire delay.
In future we plan to evaluate the delay more accurately by executing time-consuming routing.
We have added some discussions in Section~\ref{sec:conclu}.
}

\item[R3C2]
minor comments:
\begin{itemize}
    \item abstract: but a legal structure $\rightarrow$ but a valid/cost-effective structure
    \item page 10 line 31: In addition, the previous work in [13] deals with ...
\end{itemize}
\item[R3A2]\revise{
Thanks very much for the comments. We have corrected them accordingly.
}

\end{description}

}


==> doc/cover.tex <==
{
\twocolumn[
\begin{@twocolumnfalse}
\thispagestyle{empty}

Dear Editor-in-chief, Associate Editor and Reviewers,

\ \\
Thank your very much for reviewing our submission and providing your valuable comments.
\ \\

We have revised this version by addressing reviewers' comments and incorporating their suggestions.
All the recent changes in the current version are highlighted with \revise{blue} color. 


\ \\
Detailed responses to reviewers' comments are appended by the end of this manuscript.

\ \\
Best regards,

\ \\

Song Chen, Qi Xu, Bei Yu

\end{@twocolumnfalse}
]
\clearpage
%\setcounter{page}{1}
}




==> pgfplot/area.tex <==

% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{0,111,190}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7

\pgfplotsset{
    width =0.40\textwidth,
    height=0.26\textwidth
}

\begin{tikzpicture}
\begin{axis}[
xmin=1, xmax=10,
ymin=2, ymax=17,
xtick={2,3,...,10},
ytick={2,5,...,19},
xlabel=Type\ of\ MUX,
yticklabel style={/pgf/number format/fixed,/pgf/number format/precision=5},
xlabel near ticks,
ylabel={Area\ ($um^2$)},
ylabel near ticks,
legend style={
 draw = none,
 font=\footnotesize,
 at={(1.0,0.33)}
},
xticklabel={
$\pgfmathprintnumber{\tick}$\_$1$},
xtick=data,
x tick label style={/pgf/number format/fixed,/pgf/number format/precision=0},
]
\addplot [color=myblue, mark=*] coordinates {(2,2.1168) (3,3.7044) (4,4.76) (5,6.5268) (6,7.938) (7,9.8784) (8,10.584) (9,12.1716) (10,15.876)};
\end{axis}

\end{tikzpicture}


==> pgfplot/delay.tex <==

% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{0,111,190}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7

\pgfplotsset{
    width =0.40\textwidth,
    height=0.26\textwidth
}

\begin{tikzpicture}
\begin{axis}[
xmin=1, xmax=10,
ymin=0.02, ymax=0.12,
xtick={2,3,...,10},
ytick={0.03,0.05,...,0.13},
xlabel=Type\ of\ MUX,
yticklabel style={/pgf/number format/fixed,/pgf/number format/precision=3},
xlabel near ticks,
ylabel={Delay\ (\emph{ns})},
ylabel near ticks,
legend style={
 draw = none,
 font=\footnotesize,
 at={(1.0,0.33)}
},
xticklabel={
$\pgfmathprintnumber{\tick}$\_$1$},
xtick=data,
x tick label style={/pgf/number format/fixed,/pgf/number format/precision=0},
]
\addplot [color=myblue, mark=*] coordinates {(2,0.03) (3,0.05) (4,0.06) (5,0.06) (6,0.07) (7,0.1) (8,0.1) (9,0.11) (10,0.11)};
\end{axis}

\end{tikzpicture}


==> pgfplot/portnum.tex <==

% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{0,111,190}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7



\pgfplotsset{
    width =0.40\textwidth,
    height=0.26\textwidth
}
\begin{tikzpicture}
\begin{axis}[minor tick num=0,
xmin = 2,
xmax = 3,
ymin=5, ymax=9,
xticklabel style={/pgf/number format/fixed,/pgf/number format/precision=3},
xtick={2,3},
ytick={5,6,...,8},
yticklabel style={/pgf/number format/fixed,/pgf/number format/precision=0},
xlabel={$C$},
ylabel={\#Port},
xlabel near ticks,
legend style={
  draw=none,
  at={(0.50,1.23)},
  anchor=north,
  legend columns=3,
}
]
\addplot +[line width=0.7pt] [color=mylight, solid, mark=triangle]  table [x={C},  y={ami49}]  {portnum.dat};
\addplot +[line width=0.7pt] [color=red, solid, mark=o]  table [x={C},  y={n100}]  {portnum.dat};
\addplot +[line width=0.7pt] [color=blue,  solid, mark=diamond]   table [x={C},  y={n300}]  {portnum.dat};
\legend{ami49\ ,n100\ ,n300}
\end{axis}
\end{tikzpicture}


==> pgfplot/scalability.tex <==

% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{0,111,190}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7



\pgfplotsset{
    width =0.40\textwidth,
    height=0.26\textwidth
}
\begin{tikzpicture}[scale=1]
\begin{axis}[minor tick num=0,
xmin=2, xmax=8,
ymin=0, ymax=400,
xtick={3,4,...,7},
ytick={0,80,...,400},
yticklabel style={/pgf/number format/.cd, fixed, fixed zerofill, precision=3, /tikz/.cd},
xlabel={$N_{gs}$},
ylabel={RT(s)},
xlabel near ticks,
legend style={
  draw=none,
  font=\footnotesize,
  at={(0.59, 0.62)}
}
]
\addplot [color=black, mark=*]  table [x={Ngs},  y={ILP}]  {scalability.dat};
\addplot [color=myblue, mark=square*]   table [x={Ngs},  y={Heuristic}]  {scalability.dat};
\legend{\texttt{ILP} , \texttt{Heuristic}}
\end{axis}
\end{tikzpicture}


==> pgfplot/scalability1.tex <==

% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{0,111,190}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7



\pgfplotsset{
    width =0.40\textwidth,
    height=0.26\textwidth
}
\begin{tikzpicture}[scale=1]
\begin{axis}[minor tick num=0,
xmin=2, xmax=8,
ymin=0, ymax=450,
xtick={3,4,...,7},
ytick={0,90,...,450},
yticklabel style={/pgf/number format/.cd, fixed, fixed zerofill, precision=3, /tikz/.cd},
xlabel={$N_{gs}$},
ylabel={RT(s)},
xlabel near ticks,
legend style={
  draw=none,
  font=\footnotesize,
  at={(0.97, 0.42)}
}
]
\addplot [color=black, mark=*]  table [x={Ngs},  y={ILP}]  {scalability.dat};
\addplot [color=myblue, mark=square*]   table [x={Ngs},  y={Heuristic}]  {scalability.dat};
\legend{\texttt{ILP} , \texttt{Heuristic}}
\end{axis}
\end{tikzpicture}


==> pgfplot/stsvnum.tex <==

% ==== defined colors
\definecolor{myorange}{RGB}{244,106,18} %F47012
\definecolor{myblue}{RGB}{0,111,190}    %006FBE
\definecolor{mygreen}{RGB}{0,127,128}   %007F80
\definecolor{myred}{RGB}{228,46,36}     %E42E24
\definecolor{myyellow}{RGB}{198,148,34} %C69422
\definecolor{mydark}{RGB}{114,44,114}   %722C72
\definecolor{mymiddle}{RGB}{144,44,144} %902C90
\definecolor{mylight}{RGB}{167,44,167}  %A72CA7



\pgfplotsset{
    width =0.36\textwidth,
    height=0.26\textwidth
}
\begin{tikzpicture}
\begin{axis}[minor tick num=0,
xmin = 2,
xmax = 3,
ymin=60, ymax=390,
xticklabel style={/pgf/number format/fixed,/pgf/number format/precision=3},
xtick={2,3},
ytick={60,230,400},
yticklabel style={/pgf/number format/fixed,/pgf/number format/precision=0},
xlabel={$C$},
ylabel={\#s-TSV},
xlabel near ticks,
legend style={
  draw=none,
  at={(0.50,1.23)},
  anchor=north,
  legend columns=3,
}
]
\addplot +[line width=0.7pt] [color=mylight, solid, mark=triangle]  table [x={C},  y={ami49}]  {stsvnum.dat};
\addplot +[line width=0.7pt] [color=red, solid, mark=o]  table [x={C},  y={n100}]  {stsvnum.dat};
\addplot +[line width=0.7pt] [color=blue,  solid, mark=diamond]   table [x={C},  y={n300}]  {stsvnum.dat};
\legend{ami49\ ,n100\ ,n300}
\end{axis}
\end{tikzpicture}

